What You See is What You Get: Principled Deep Learning via Distributional Generalization

Having similar behavior at training time and test time $-$ what we call a "What You See Is What You Get" (WYSIWYG) property $-$ is desirable in machine learning. Models trained with standard stochastic gradient descent (SGD), however, do not necessarily have this property, as their complex behaviors such as robustness or subgroup performance can differ drastically between training and test time. In contrast, we show that Differentially-Private (DP) training provably ensures the high-level WYSIWYG property, which we quantify using a notion of distributional generalization. Applying this connection, we introduce new conceptual tools for designing deep-learning methods by reducing generalization concerns to optimization ones: to mitigate unwanted behavior at test time, it is provably sufficient to mitigate this behavior on the training data. By applying this novel design principle, which bypasses "pathologies" of SGD, we construct simple algorithms that are competitive with SOTA in several distributional-robustness applications, significantly improve the privacy vs. disparate impact trade-off of DP-SGD, and mitigate robust overfitting in adversarial training. Finally, we also improve on theoretical bounds relating DP, stability, and distributional generalization.

==> app-calibration.tex <==
\section{Calibration Generalization via Strong Distributional Generalization}
\label{app:calibration}

For simplicity we consider binary classifiers, 
with $\sY = \{0, 1\}$ and $f_\theta:  \sX \to [0, 1]$.

The \emph{calibration gap}, or Expected Calibration Error (ECE), of a classifier $f_\theta$ is
defined as:
\begin{align*}
\cgap(f_\theta)
&:=
\E\left[\left\vert \E[y \mid f_\theta(x) ] - f_\theta(x) \right\vert\right]\\
&=
\int_{0}^1
\left\vert
\E\left[
y - p
\mid f_\theta(x) = p
\right]
\right\vert
d F(p)
\tag{where $F(p)$ is the law of $f_\theta(x)$}\\
\end{align*}
Where all expectations are taken w.r.t. $(x, y) \sim \datagen$.
To estimate this quantity from finite samples, we will discretize the interval $[0,1]$. The \emph{$\tau$-binned calibration gap} of a classifier $f_\theta$ is:
\begin{align*}
\cgap_\tau(f_\theta; \datagen) &:=
\sum_{p \in \{0, \tau, 2\tau, \dots, 1\}}
\left\vert
\E_{(x, y) \sim \datagen}\left[
\1\{f_\theta(x) \in (p, p+\tau)\}
\cdot
(y - p)
\right]
\right\vert
\end{align*}
So that $\cgap_\tau \to \cgap$ as the bin width $\tau \to 0$.
The empirical version of this quantity, for train set $S$, is:

\begin{align*}
\cgap_\tau(f_\theta; S) &:=
\sum_{p \in \{0, \tau, 2\tau, \dots, 1\}}
\left\vert
\E_{x, y \sim S}\left[
\1\{f_\theta(x) \in (p, p+\tau)\}
\cdot
(y - p)
\right].
\right\vert
\end{align*}


We will now show that the strong Distributional Generalization (Definition \ref{def:strong-dg}) implies 
that the expected binned calibration gap is similar between train and test.

\begin{theorem}
If the training method $\theta$ satisfies $\delta$-strong DG, then
\begin{equation*}
\left| \E_{\theta, S\sim\mathcal{D}^n} \cgap_{\tau}(f_{\theta(S)}; S) - \cgap_{\tau}(f_{\theta(S)}; \mathcal{D})\right| \leq \frac{\delta}{\tau}.
\end{equation*}
\end{theorem}
\begin{proof}
First, let us define the family of tests:
\begin{align*}
\phi_p(x,y; \theta)
:= 
\1\{f_\theta(x) \in (p, p+\tau)\}
\cdot
(y - p)
\end{align*}
The assumed $\delta$-strong DG implies that each of these tests $\phi_p$ have similar expectations between
train and test distributions:
\begin{align*}
\forall p
\left|
\E_{S \sim \datagen^n; (x, y) \sim S}[
\phi_p(x,y; \theta(S))
]
-
\E_{S \sim \datagen^n; (x, y) \sim \datagen}[
\phi_p(x,y; \theta(S))
]
\right|
\leq \delta
\end{align*}

Thus, the difference in expected calibration gaps between train and test is:
\begin{align*}
&
|\E_{S \sim \datagen^n}[
\cgap_\tau(f_\theta; S)
-
\cgap_\tau(f_\theta; \datagen) 
]|\\
&=
\left|
\E_{S \sim \datagen^n}
\sum_{p \in \{0, \tau, 2\tau, \dots, 1\}}
\left|\E_{x, y \sim S}[\phi_p(x, y; \theta)]\right|
-
\left|\E_{x, y \sim \datagen}[\phi_p(x, y; \theta)]\right|
\right|\\
&\leq
\sum_{p \in \{0, \tau, 2\tau, \dots, 1\}}
\E_{S \sim \datagen^n}
\left|\E_{x, y \sim S}[\phi_p(x, y; \theta)
-
\E_{x, y \sim \datagen}[\phi_p(x, y; \theta)]
\right|\\
&\leq
\frac{\delta}{\tau},
\end{align*}
where the last inequality follows from the definition of $\delta$-strong DG applied to functions $\phi_p$.
\end{proof}

==> app-other_dg.tex <==
\section{Other Methods That Achieve DG}

As mentioned in \cref{sec:algorithms}, many regularization methods can be used to improve different generalization gaps.
For example, \citet{sagawa2019distributionally} show that strong $\ell_2$ regularization helps with improving group-distributional generalization, and \citet{YY2020roblocallip} show that dropout helps with adversarial-robustness generalization.
However, these works do not have theoretical justification.
In \cref{fig:other_dg_methods}, we show the training and testing worst-group accuracy with different strength of $\ell_2$ regularization and on different epochs (w/ and w/o $\ell_2$ regularization).
We have three observations:
(1) with properly tuned regularization parameter, the gap between training and testing worst-group accuracy can be narrowed,
(2) the gap can start widening in very early stage of training, and
(3) the testing worst-group accuracy can fluctuate largely, which highlights the importance of using validation set for early stopping in this task.

\begin{figure}[h!]
    \centering
    \subfigure[CelebA]{\includegraphics[width=.3\textwidth]{images/regularizations/l2reg_celebA.pdf}}
    \subfigure[UTKFace]{\includegraphics[width=.3\textwidth]{images/regularizations/l2reg_utkface.pdf}}
    \subfigure[iNat]{\includegraphics[width=.3\textwidth]{images/regularizations/l2reg_inaturalist.pdf}}
    
    \subfigure[CelebA (no reg.)]{
      \includegraphics[width=.3\textwidth]{images/regularizations/earlystop_celebA.pdf}}
    \subfigure[UTKFace (no reg.)]{
      \includegraphics[width=.3\textwidth]{images/regularizations/earlystop_utkface.pdf}}
    \subfigure[iNat (no reg.)]{
      \includegraphics[width=.3\textwidth]{images/regularizations/earlystop_inaturalist.pdf}}
    
    \subfigure[CelebA ($\ell_2$ reg.)]{
      \includegraphics[width=.3\textwidth]{images/regularizations/earlystop_celebA-wd.pdf}}
    \subfigure[UTKFace ($\ell_2$ reg.)]{
      \includegraphics[width=.3\textwidth]{images/regularizations/earlystop_utkface-wd.pdf}}
    \subfigure[iNat ($\ell_2$ reg.)]{
      \includegraphics[width=.3\textwidth]{images/regularizations/earlystop_inaturalist-wd.pdf}}
    
    \caption{
    We show the training and testing worst-group accuracy with different strength of $\ell_2$ regularization and on different epochs (w/ and w/o $\ell_2$ regularization).
    The network is trained with \iserm on CelebA, UTKFace, and iNat.
    For (a), (b), and (c), we show the result of the last epoch.
    For (g), (h), and (i), we set weight decay to $0.01$.
    }
    \label{fig:other_dg_methods}
\end{figure}
